RNNs Implicitly Implement Tensor Product Representations

Recurrent neural networks (RNNs) can learn continuous vector representations of symbolic structures such as sequences and sentences; these representations often exhibit linear regularities (analogies). Such regularities motivate our hypothesis that RNNs that show such regularities implicitly compile symbolic structures into tensor product representations (TPRs; Smolensky, 1990), which additively combine tensor products of vectors representing roles (e.g., sequence positions) and vectors representing fillers (e.g., particular words). To test this hypothesis, we introduce Tensor Product Decomposition Networks (TPDNs), which use TPRs to approximate existing vector representations. We demonstrate using synthetic data that TPDNs can successfully approximate linear and tree-based RNN autoencoder representations, suggesting that these representations exhibit interpretable compositional structure; we explore the settings that lead RNNs to induce such structure-sensitive representations. By contrast, further TPDN experiments show that the representations of four models trained to encode naturally-occurring sentences can be largely approximated with a bag of words, with only marginal improvements from more sophisticated structures. We conclude that TPDNs provide a powerful method for interpreting vector representations, and that standard RNNs can induce compositional sequence representations that are remarkably well approximated by TPRs; at the same time, existing training tasks for sentence representation learning may not be sufficient for inducing robust structural representations.

==> backup.tex <==
\footnote{Although LSTMs \citep{hochreiter1997long} have also achieved great successes in sequence processing , we chose GRUs because they make use of a single internal state for their representations, making their representations more straightforward to analyze than those of LSTMs, which use two internal states (the hidden state and the cell state).} 

\section{Lit review}

\cite{adi2017fine}: Classification tasks to analyze representations. 
\begin{itemize}
\item Sentence representations do pretty well at probing tasks investigating the length of the sentence, word order in the sentence, and whether a given word is present in the sentence. A TPR would be expected to succeed at all of these.
\item At the same time, they don't do great (it's roughly 80\%). So maybe the reason they only do ok is because the models have not learned a robust tensor product representation.
\item Also of note: BOW models do well at word order prediction, indicating that statistical regularities in English might make many tasks not really require representations of structure.
\end{itemize}

\cite{ettinger2018assessing}: Probing tasks for vector representations.
\begin{itemize}
\item Similar takeaways as above: These probing tasks would be handled perfectly, or near-perfectly, by a TPR.
\end{itemize}


\cite{vaswani2017attention}: not sure we need that

Something about the kernel trick and how it makes nonlinearities unnecessary? (I don't know much about this, but my impression is that if you define the proper kernel, things become linearly separable that weren't before, making a nonlinearity unnecessary. So perhaps using a certain role scheme also plays a similar role).\todotl{Interesting but I don't fully see it so I suggest taking out.}
\subsection{Speech}

I have obtained some pretrained acoustic word embeddings from the author of a paper on such things. The embeddings were trained on a task of, given 2 recordings (word A and word B), determining whether word A and word B are the same utterance. So the embeddings should encode phonetic similarity in some sense, so I plan to see if they can be decomposed with phonemes as fillers (probably by just looking up the words in the CMU pronouncing dictionary) and linear positions as fillers.

\subsection{Vision}

I have gotten 2 pretrained computer vision models working in PyTorch (Alexnet and Resnet) such that I can plug in any image and get the embedding for that image from the models.

I have two ideas for proceeding here:
\begin{enumerate}
\item \textbf{CLEVR:} Use the CLEVR dataset, with the hypothesis that an image can be decomposed with the shapes being fillers and their positions being roles. (A little tricky because the positions vary continuously--so will either need to bin or to have continuously-valued roles). Might also be able to further decompose shape representations based on shape, color, size, etc.
\item \textbf{MNIST:} Use the MNIST dataset, with the hypothesis that an image can be decomposed with the pixels being roles and the darknesses/hues of the pixels being fillers.
\end{enumerate}



\section{Submission of conference papers to ICLR 2019}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2019 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available on the World Wide Web at
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2019_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2019_conference.sty+ and \verb+iclr2019_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2019_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis (as in ``Deep learning shows promise to make progress towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.


\subsubsection*{Acknowledgments}

Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

\section{The Decomposition Architecture}

Points: 
\begin{itemize}
\item Different architectures have different role schemes that work: Linear positions for unidirectional, tree positions for tree structured; bidirectional doesn't work very well.
\item The decoder seems to be what really determines it. "Accommodating encoder" hypothesis. E.g., with uni/tree, the encoder basically learns to parse; but with tree/uni, the decoder isn't learning to read a parse; rather, the encoder is learning to linearize the tree.
\item Not perfect, though: Tree/Uni is still better fit by tree roles than uni/uni and bi/uni are.
\item Task plays a role too: For both autoencode and reverse, Uni/Uni is "mildly bidirectional", but the unidirectional version that approximates the bidirectional best varies (ltr for autoencode, rtl for reverse). In addition, rtl is better for reverse than ltr is for autoencode; maybe partly explains why reversal helps with seq2seq. Then for interleave, uni/uni is properly (not mildly) bidirectional. 
\item For sort, you get BOW roles (so of course others work too); except for with a tree decoder, where you still need to represent the tree.
\item The emergence of bidirectionality
\end{itemize}



==> delete.tex <==

\section{Applications to existing models}

Here we investigate how this approach can be used to study five distinct, structured spaces: Sentences, word meanings, abstract syntactic structures, sound waves, and images.

\subsection{Sentences}

\subsubsection{Models}

We investigate 3 preexisting models for embedding sentences:

\begin{itemize}
\item InferSent \citep{conneau2017supervised}
\item Skip-thought \citep{kiros2015skip}: Trained on predicting neighboring sentences; LSTM-based. 2400 dimensions. So far I've only used one version of it, but there are others easily accessible.
\item Stanford CoreNLP recursive sentiment predictor \citep{socher2013recursive}: Trained on autoencoding (sort of) and sentiment analysis; Tree-RNN-based. 25 dimensions.
\end{itemize}

\textbf{Hypotheses:} The LSTM-based architectures will be decomposable with linear-index roles. The recursive architecture will be decomposable with tree-position roles.

\subsubsection{Experiment 1}

\textbf{Corpus:} SNLI \citep{bowman2015large}. For each model, we pass all SNLI train and test premises through the model to get a vector representing the sentence. [NOTE: I used SNLI because at first I was just thinking about InferSent. But it might be a weird thing to use just as a text corpus given that I have other models now--maybe switch to Wikipedia?]

\textbf{The TPR model:} I assume that the words are the fillers. It is not feasible to train new filler embeddings for all the fillers due to data sparsity; instead, I just use the word embeddings that each model uses:
\begin{itemize}
\item InferSent: fasttext
\item Skip-thought: Has its own embeddings (but for the experiment reported below I actually use fastText; am working on extracting the Skip-thought word embeddings for use here).
\item Stanford: Has its own embeddings
\end{itemize}
But I do train role embeddings and the final linear layer. For InferSent and Skip-thought, I assume that linear indices are the roles. For Stanford, I assume the tree positions are roles. [TODO--Test more roles as controls, and in general add controls to the applied experiments.]. 

\textbf{Training:} I train the TPR model to take in a sentence from the SNLI training set and to map it to the vector for that sentence generated by InferSent/Skip-thought/Stanford. 

\textbf{Evaluation:} I use the trained TPR model to embed all the sentences from the SNLI test set. For each of these embeddings, I then take the Euclidean distance between it and each SNLI test set vector generated by InferSent/SkipThought/Stanford. I compute two measures of success: average rank (the average position of the correct sentence in an ordered ranking of all test vectors by smallest Euclidean distance) and accuracy (the proportion of test sentences for which the top-ranked candidate was the correct one). [TODO--also include MSE, along with controls to help interpret it]

\textbf{Results:} WARNING: SkipThought is actually using a different set of sentences than the others.


\begin{tabular} {ccc} \toprule
Model & Avg. rank & Acc. \\ \midrule
InferSent & 1.22 & 0.999 \\
Skip-thought & 11.34 & 0.814 \\
Stanford & 78.62 & 0.078 \\ \midrule
Chance & 439 & 0.001 \\ \bottomrule
\end{tabular}

\textbf{Possible extensions:} See if these models still perform comparably at their own tasks using the TPRs instead of the models' encoders.

\subsubsection{Experiment 2}

One possible objection to Experiment 1 is that, since it uses naturalistic sentences, no two sentences in the corpus are going to be very similar. Thus, the task of discriminating between two sentences might be overly easy and accomplishable with only a very coarse-grained approximation of the model. Experiment 2 addresses that complaint by using a very systematic dataset replete with minimal pairs.

\textbf{Corpus:} I construct a set of sentences where each is 5 words long, fitting the following template: \textit{The NOUN VERBED the NOUN.} For the nouns and verbs, I use the lexical items from \cite{ettinger2018assessing}, which insures that the resulting sentences will all be plausible. Their lexicon has 16 verbs and 34 nouns (17 lemmas with both singular and plural forms), making for 18,496 sentences total. Examples would be: \textit{The assistant advised the lawyer}, \textit{The men supported the student}, \textit{The judges followed the bankers}...

\textbf{The TPR model:} Same as before (words = fillers, linear positions = roles). However, now that there is such a restricted lexicon, it is possible to train embeddings anew, so I do so.

\textbf{Results:} 


\begin{tabular} {ccc} \hline
Model & Avg. rank & Acc. \\ \hline \hline
InferSent & 1.0 & 1.0  \\
Skip-thought & 1.0 & 1.0 \\
Stanford &  17.5 & 0.210 \\ \hline
Chance & 925 & 0.0005 \\ \hline
\end{tabular}

\section{How does the architecture affect the learned representation?}

We train several architectures on the task of autoencoding. Each architecture is an encoder-decoder framework; we test 3 types of encoders (unidirectional bidirectional, and tree-based) and 2 types of decoders (unidirectional and tree-based) for a total of six  architectures. For the tree-based architectures, the trees were generated with an algorithm that deterministically creates a tree for any sequence of digits:

\textbf{Parsing strategy:} At each timestep, combine the smallest element of the sequence (other than the last element) with its neighbor immediately to the right, and replace the pair with that neighbor. If there is a tie for smallest, choose the leftmost one. \begin{itemize}
\item 5 2 3 7 1 9 8
\item 5 2 3 7 [1 9] 8
\item 5 [2 3] 7 [1 9] 8
\item 5 [ [2 3] 7] [1 9] 8
\item $[$ 5 [ [2 3] 7] [1 9] ] 8
\item $[$ [5 [ [2 3] 7] [1 9] ] 8]
\end{itemize}

Table \ref{tab:auto_acc} shows the performance of these architectures at their training task. All perform well, though there is always an advantage for architectures for which both the encoder and decoder belong to the same class (i.e. either both linear or both tree-based).

We then attempt to fit a TPR network onto the trained autoencoder. For each autoencoding architecture, we test six different role schemes, enumerated here:

\begin{itemize}
\item Bag of words (BOW): There is only one role, which all fillers have.
\item Left-to-right indices (LTR): A filler's role is its index in the sequence, counting from left to right.
\item Right-to-left indices (RTL): A filler's role is its index in the sequence, counting from left to right.
\item Bidirectional indices (FB): A filler's role is a 2-tuple specifying its distance from the left edge and its distance from the right edge.
\item Contextual roles (Wickel): A filler's role is a 2-tuple indicating its left neighbor and its right neighbor.
\item Tree-based roles (Tree): A filler's role is its position in the tree.
\end{itemize}

Table \ref{tab:arch} shows the results. Architecture does have an effect on learned representations. Both fully linear architectures were best fit with linear roles, while the only fully tree-based architecture was best fit with tree-based roles. Note that, for both linear ones, LTR significantly outperforms RTL.

The question might arise: Is the representation determined by the encoder, the decoder, or both? The bottom half of the table suggests that both play an effect.

\begin{table}
\centering
\begin{tabular} {ccc} \toprule
& Linear decoder & Tree decoder \\ \midrule
Linear encoder & 0.996 & 0.967 \\
Bidirectional encoder & 0.981 & 0.957 \\
Tree encoder & 0.876 & 0.985 \\ \bottomrule
\end{tabular}
\caption{Accuracies of the various architectures at the autoencoding task.}\label{tab:auto_acc}
\end{table}

\begin{table}
\centering
\begin{tabular} {ccccccc} \toprule
Architecture & BOW & LTR & RTL & FB & Wickel & Tree \\ \midrule
Linear/Linear & 0.004  & 0.812  & 0.205 & \textbf{0.936} & 0.159 & 0.245 \\
Bidirectional/Linear & 0.005  & 0.731 & 0.179 & \textbf{0.800} & 0.151 & 0.203 \\
Tree/Tree* & 0.057  & 0.332 & 0.500 & 0.544 & 0.571 & \textbf{0.891} \\
Linear/Tree & 0.035 & 0.429 & 0.609 & 0.679 & 0.619 & \textbf{0.776} \\
Bidirectional/Tree & 0.032  & 0.458 & 0.637 & 0.721 & 0.609 & \textbf{0.755} \\
Tree/Linear* & 0.007 & 0.322 & 0.237 & 0.458 & 0.245 & \textbf{0.527}\\ \bottomrule
\end{tabular}
\caption{Accuracy at decoding from a tensor-product approximation of the original encoder.} \label{tab:arch}
\end{table}

TODO: Add in controls (shuffled vectors, random encoder)

TODO: This parsing algorithm is like Berber syllabification--tftkt.

Maybe add random trees along with systematic trees

\section{How does the training task affect the learned representation?}

Maybe take out Wickelroles; maybe replace each pair with the smaller of the two pairs. (Might be similar to tree thing).

We now investigate how the training task affects the learned representations. [Maybe just focus on one architecture here, e.g. BiRNN]. We use 4 training tasks:

\begin{itemize}
\item Autoencoding
\item Sequence reversal
\item Sorting (returning the sequence in order from smallest to largest)
\item Interleaving (alternately outputting from the left and from the right; e.g. [3,4,8,1,9,2,7] -> [3,7,4,2,8,9,1])
\end{itemize}

Table \ref{tab:tasks} shows the results on these tasks for various architectures. Tables 4-6 show the results for fitting various tensor product representations onto these trained networks. When only looking at the top-ranked role scheme, little seems to change. However, a more detailed analysis does reveal changes:

For both linear models, the bidirectional roles are best for both autoencoding and reversal, but only by a relatively narrow margin; and the thing that is in close second place depends on the task.

For sorting, a bag of words representation seems natural; however, the bias for the tree RNN to use a tree-based architecture must be so strong that it overcomes the push to use a bag of words.

Meanwhile, for Interleave, a bidirectional scheme seems most natural: Whereas, for autoencoding and reversal the bidirectional scheme was only narrowly winning, here it is the clear standout. (Try tree encoder and linear decoder)

\begin{table}
\centering
\begin{tabular} {ccccc} \toprule
Architecture & Autoencode & Reverse & Sort & Interleave \\ \midrule
Linear/Linear & 0.996 & 0.992 & 0.999 & 0.997 \\
Bidirectional/Linear & 0.981 & 0.984 & 0.999 & 0.997 \\
Tree/Tree & 0.985 & 0.957 & 0.998 & 0.903 \\ \bottomrule
\end{tabular}
\caption{Accuracies on the training tasks} \label{tab:tasks}
\end{table}

\begin{table}
\centering
\begin{tabular} {ccccccc} \toprule
Task & BOW & LTR & RTL & FB & Wickel & Tree \\ \midrule
Autoencode & 0.004 & 0.812 & 0.205 & \textbf{0.936} & 0.159 & 0.245 \\
Reverse & 0.004 & 0.144 & 0.868 & \textbf{0.917} & 0.035 & 0.248 \\
Sort & \textbf{0.912} & 0.902 & 0.901 & 0.909 & 0.127 & 0.769 \\
Interleave & 0.003 & 0.305 & 0.195 & \textbf{0.957} & 0.241 & 0.321 \\ \bottomrule
\end{tabular}
\caption{Results for the Linear/Linear architecture}
\end{table}

\begin{table}
\centering
\begin{tabular} {ccccccc} \toprule
Task & BOW & LTR & RTL & FB & Wickel & Tree \\ \midrule
Autoencode & 0.005 & 0.731 & 0.179 & \textbf{0.800} & 0.151 & 0.203 \\
Reverse & 0.004 & 0.168 & 0.763 & \textbf{0.857} & 0.094 & 0.244  \\
Sort & 0.919 & 0.918 & 0.920 & \textbf{0.928} & 0.525 & 0.778  \\
Interleave & 0.005 & 0.331 & 0.158 & \textbf{0.990} & 0.432 & 0.301  \\ \bottomrule
\end{tabular}
\caption{Results for the Bidirectional/Linear architecture}
\end{table}

\begin{table}
\centering
\begin{tabular} {ccccccc} \toprule
Task & BOW & LTR & RTL & FB & Wickel & Tree \\ \midrule
Autoencode & 0.057 & 0.332 & 0.500 & 0.544 & 0.571 &  \textbf{0.891} \\
Reverse & 0.002 & 0.148 & 0.200 & 0.422 & 0.377 & \textbf{0.651}  \\
Sort & 0.266 & 0.415 & 0.475 & 0.503 & 0.507 & \textbf{0.937}  \\
Interleave & 0.003 & 0.104 & 0.120 & 0.265 & 0.296 & \textbf{0.484}  \\ \bottomrule
\end{tabular}
\caption{Results for the Tree/Tree architecture}
\end{table}

TODO: Add in controls (shuffled vectors, random encoder)

\section{Interchangeability?}

Can these models learn each other's representations?

\section{Model details}

TODO:
\begin{itemize}
\item What dimension of roles and fillers is correct? (heatmap)
\item How does the final linear layer affect things?
\item What if you don't dictate the set of roles? (role learning)
\end{itemize}




\section{Experiment 1: Digit Sequences}

We first test these hypotheses in a controlled setting, with an artificial language. 

\subsection{Language}

The language consisted of sequences of digits. The sequences varied in length from 1 to 6, and the possible digits used were the digits from 0 to 9. We generated 50,000 unique sequences within these constraints, split into 40,000 training examples, 5,000 development examples, and 5,000 test examples.

\subsection{Architectures}

All experiments used variations of an encoder/decoder, sequence-to-sequence framework \citep{sutskever2014sequence} with recurrent neural networks (RNNS) \citep{elman1990finding}. For the recurrent units, we used gated recurrent units (GRUs) \citep{cho2014learning}; though long short-term memory units (LSTMs) \citep{hochreiter1997long} are also popular, we chose GRUs because GRUs make use of a single hidden state for their representations, making their representations more straightforward to analyze than those of LSTMs, which use two hidden states (known as the hidden state and the cell state).

For both the encoders and the decoders, we tested three basic types of architectures: unidirectional, bidirectional, and tree-based. These are depicted in Figure FIG. 

Encoders:
Unidirectional RNNs are the most standard sort, following the basic structure of \cite{elman1990finding}. Bidirectional RNNs \citep{schuster1997bidirectional} involve two unidirectional RNNs, one that processes the input from left to right and another that processes the input from right to left; the final encoding of the sequence is then derived by concatenating the encoding from the forward encoder and the encoding from the backward encoder. Tree-based RNNs \citep{pollack1990recursive,socher2010learning} compose encodings of an entire sequence based on a tree structure; we specifically use the Tree-GRU of \cite{chen2017improved}.

Decoders:
The unidirectional decoder is very similar to the unidirectional decoder, but instead of receiving one digit as input at each time stop it outputs one digit at each timestep. This is by far the most standard type of decoder, but to explore how different architectures affect the learned representations, and for parallelism with the encoders, we also consider two other types of decoders: bidirectional and tree based. The bidirectional decoder consists of two separate unidirectional decoders (a forward decoder and a reverse decoder), each of which receives the encoding as input and then generates a list of $n$ hidden states, where $n$ is the length of the sequence. The output word at position $i$ is then generated by first concatenating the $i$th hidden state of the forward decoder with the $n-i$th hidden state of the reverse decoder to create the complete $i$th hidden state; as with the other decoders, this hidden state is then passed through a linear layer and a softmax to choose the output element. For the tree decoder, we use the binary tree decoder from \cite{chen2018tree}; this architecture works by having two separate recurrent units, which we will call GRU$_L$ and GRU$_R$ for left and right. For a parent node $h$, the hidden states of its left and right child are generated by applying either GRU$_L$ or GRU$_R$ to the hidden state of $h$, respectively. In this way, a binary tree is built following a pre-defined tree structure; the output words are then generated from the leaf nodes of the tree.

For all decoders, when computing a new hidden state, the only input to the recurrent unit is another hidden state. This property is necessary to allow the bidirectional encoder to be defined as it is here. We also provide the decoder with the length of the output; it generates output words until this length is reached and then stops (or, in the case of the tree decoder, we provide it with the tree, which it uses to generate output and then stops). Stopping can alternately be determined by some action of the decoder (e.g. generating an end-of-sequence symbol) but for simplicity we indicated the sequence length instead.


\subsection{Parameters and Training}

For all architectures, we used an embedding dimensionality of 10 (chosen arbitrarily) and a hidden size of 60 (this hidden size was chosen because 60 has many integer factors, making it amenable to the analysis in Section SECTION). For the bidirectional architectures, the forward and reverse recurrent units each had a hidden size of 30, so that their concatenated hidden size was then 60. For bidirectional decoders, a linear layer condensed the 60-dimensional encoding into 30 dimensions before it was passed to the forward and reverse decoders. The networks were trained using the Adam optimizer \citep{kingma2015adam} with the standard initial learning rate 0f 0.001. We used negative log likelihood, computed over the softmax probability distributions for each output sequence element, as the loss function. Training proceeded with a batch size of 32, with loss on the heldout development set computed after every 1,000 training examples.  Training was halted when the loss on the heldout development set had not improved for any of the development loss checkpoints for a full epoch of training (i.e. 40,000 training examples). Once training completed, the parameters from the best-performing checkpoint were reloaded and used for evaluation of the network. 

\subsection{Experiment 1: Effect of the architecture}

We first investigate the effect that the architecture has on the representations that are learned. We trained one network for each of the 3 types of encoders and 3 types of decoders, for 9 architectures total. In all cases, these networks were trained on the task of autoencoding (returning the same sequence that was provided as input). We then attempted to decompose the learned representation into fillers and roles using each of the role schemes provided in Figure FIG. To control for the effects of random initialization, we ran each experiment 5 times with different random initializations and averaged the results.

Results:
Results are shown in Figure FIG. They show that...



\subsection{Effect of task}

As Marr points out, both Arabic numerals and Roman numerals are equivalent, yet multiplication is straightforward using Arabic numerals but difficult using Roman numerals. Binary and decimal numbers are equivalent; but with decimal numbers it is trivial to tell if the number is a power of 10 and hard to tell if a power of 2, while for binary it is reversed.

if one chooses the Arabic numeral representation, it is easy to discover whether a number is a power of 10 but difficult to discover whether it is a power of 2. If one chooses the binary representation, the situation is reversed

Shuffling baseline

\subsection{Generalize to longer seqs?}

\subsection{Removing the final linear layer}

\subsection{Varying the embedding size}

\section{Experiment 2: Sentence Embeddings}

\subsection{The models}

\subsection{The corpora}

\subsection{Results}

Performance on downstream tasks

\subsection{Investigating the learned role embeddings}

\subsection{Can we unbind?}

\subsection{Can we do analogies?}

\subsection{Other combination methods}

\subsection{Linear transform of GloVe embeddings}

\subsection{Role learning}

\subsection{As a speedup}

\subsection{To improve models}

\subsection{Comparison to other models/techniques}

\begin{tabular} {ccccc}
    \toprule
Model & Topology & Training task & Hidden size & Word embeddings \\ \midrule
InferSent & BiLSTM & SNLI & 4096 & FastText \\
Skip-thought & LSTM & Skip-thought & 2400 & Transformed word2vec \\
SST & RNTN & Sentiment labeling & 25 & Learned \\
SPINN & TreeLSTM & SNLI & 300 & GloVe \\ \bottomrule
\end{tabular}


\floatsetup[figure]{style=plain,subcapbesideposition=top}
\begin{figure}
  \sidesubfloat[]{\includegraphics[scale=0.2]{tpr_architecture.pdf}}\quad%
  \sidesubfloat[]{\includegraphics[scale=0.5]{tensor_product.pdf}}%
  \caption{(a) The tensor product decomposition architecture. (1) The fillers and roles are embedded. (2) The fillers and roles are bound together using the tensor product. (3) The tensor products are summed. (4) The sum is flattened into a vector by concatenating the rows. (5) A linear transformation is applied to get the final encoding. (b) An example of the tensor product operation.}\label{fig:arch}
\end{figure}

\begin{table} \label{tab:tasks}
\centering
\caption{Examples for each training task}
\begin{tabular} {ccc} \toprule
Input & 34097 & 436513 \\ \midrule
Autoencoding & 34097 & 436513 \\
Reversal & 79043 & 315634 \\
Sorting & 03479 & 133456 \\
Interleaving & 37490 & 433165 \\ \bottomrule
\end{tabular}
\end{table}


\begin{table} \label{tab:taskacc}
\centering
\caption{Substitution accuracy for various tasks. Each number is an average across five random intializations.}
\begin{tabular} {cccccccc}
    \toprule
Task & LTR & RTL & Bi & Wickel & Tree & BOW \\ \midrule
Autoencode & 0.87 & 0.11 & \textbf{0.99} & 0.28 & 0.25 & 0.00 \\ 
Reverse & 0.06 & 0.99 & \textbf{1.0} & 0.18 & 0.20 & 0.00 \\ 
Sort & 0.90 & 0.90 & \textbf{0.92} & 0.88 & 0.89 & 0.89 \\
Interleave & 0.27 & 0.18 & \textbf{0.99} & 0.63 & 0.36 & 0.00 \\ \bottomrule

\end{tabular}
\end{table}





\begin{table}
\centering
\begin{tabular} {ccccccc}
Model & LTR & RTL & Bi & Tree & BOW \\ \hline
InferSent & \textbf{0.79} & \textbf{0.79} & 0.78 & 0.78 & 0.77\\
Skip-thought &  0.53 & 0.52 & 0.46 & 0.50 & \textbf{0.58} \\
SST & \textbf{0.83} & 0.82 & 0.82 & 0.82 & 0.81\\
SPINN & 0.73 & 0.75 & 0.75 & \textbf{0.76} & 0.74  \\ \hline
\end{tabular}
\caption{Other agreements averaged} \label{tab:other_agr}
\end{table}

\begin{table}
\centering
\begin{tabular} {ccccccc}
Model & LTR & RTL & Bi & Tree & BOW \\ \hline
InferSent & \textbf{0.77} & 0.74 & \textbf{0.77} & \textbf{0.77} & 0.71 \\
Skip-thought & \textbf{0.37} & \textbf{0.37} & 0.36 & 0.36 & \textbf{0.37}  \\
SST & 0.48 & 0.51 & 0.49 & \textbf{0.67} & 0.49  \\
SPINN & 0.72 & 0.72 & 0.73 & \textbf{0.76} & 0.58  \\ \hline
\end{tabular}
\caption{SNLI agreements.} \label{tab:snli_agr}
\end{table}


\begin{table} 
\centering
\caption{\label{tab:analogydist}Euclidean distances (lower is better)}
    \resizebox{\textwidth}{!}{
        \begin{tabular} {cccccc|c}
\toprule
Model & LTR/BOW & RTL/BOW & LTR/RTL/Bi/Tree/BOW & Tree/BOW & BOW & Chance \\ \midrule
InferSent & 0.91 & 0.90 & \textbf{0.66} & 0.92 & 1.14 & 2.30 \\
Skip-thought & 0.40 & 0.44 & \textbf{0.22} & 0.39 & 0.84 & 0.90 \\
SPINN & 5.41 & 6.08 & \textbf{4.34} & 5.34 & 6.56 & 9.96 \\
SST & 0.25 & 0.33 & \textbf{0.22} & 0.23 & 0.45 & 0.88 \\ \bottomrule
\end{tabular}
}
\end{table}

\begin{table} 
\centering
\caption{\label{tab:analogycos}Cosine (higher is better)}
    \resizebox{\textwidth}{!}{
\begin{tabular} {ccccccc|c}
\toprule
Model & LTR/BOW & RTL/BOW & LTR/RTL/Bi/Tree/BOW & Tree/BOW & BOW & Chance \\ \midrule
InferSent & 0.92 & 0.92 & \textbf{0.95} & 0.92 & 0.88 & 0.46 \\
Skip-thought & 0.96 & 0.95 & \textbf{0.99} & 0.96 & 0.84 & 0.80 \\
SPINN & 0.89 & 0.86 & \textbf{0.93} & 0.89 & 0.84 & 0.59 \\
SST & 0.93 & 0.89 & \textbf{0.94} & \textbf{0.94} & 0.82 & 0.36 \\ \bottomrule
\end{tabular}
}
\end{table}



%\begin{table}
%\centering
%\setlength{\tabcolsep}{3pt}
%\begin{tabular} {l rr rr rr rr rr rr}
%    \toprule
%   & \multicolumn{2}{c}{LTR} & \multicolumn{2}{c}{RTL} & \multicolumn{2}{c}{Bi}  & \multicolumn{2}{c}{Tree} & \multicolumn{2}{c}{BOW} \\ \midrule
%    InferSent & 997 & (5.6) & 986 & (206) & 985 & (554) & 992 & (7.3) & 989 & (284) \\
%    Skip-thought & 3 & (36004) & 2 & (41607) & 0 & (47444) & 1 & (29300) & 2 & (36509) \\
%    SST & 0 & (29004) & 0 & (33752) & 1 & (32250) & 1 & (14702) & 0 & (36135) \\
%    SPINN & 848 & (175) & 850 & (331) & 842 & (519) & 936 & (40) & 752 & (552) \\ \bottomrule
%\end{tabular}
%\caption{Nearest neighbor results: For each model, we report the number correct out of 1,000 and the average rank of the correct answer in parentheses.} \label{tab:neighbor}
%\end{table}

%\paragraph{Nearest neighbor evaluation} Mean squared error is not very interpretable on an absolute level. Therefore, we next introduce the nearest neighbor metric, defined as follows: For a given sentence in the test set, encode it as a vector using the tensor product approximation. Then, check its Euclidean distance from the vector encodings of all sentences in the original dataset (training, development, and testing) and see if the nearest neighbor of the vector is the correct sentence. Table \ref{tab:neighbor} shows the results.


\subsubsection{Bidirectional roles in a unidirectional network}

It may seem surprising that the unidirectional architecture appears to utilize bidirectional roles. It is well established that unidirectional RNNs can keep track of left-to-right position (CITE), but how can it incorporate right-to-left information into its representation when it only processes the information left-to-right?

Consider a simplified RNN consisting of a simple recurrent network \cite{elman1990finding} with no nonlinearities or bias term; that is, with a hidden state update defined as:

\begin{equation}
h_{t} = Wh_{t-1} + Ux_t
\end{equation}

In this simple case, if we assume the hidden state is initialized with zeros, we can equivalently write [does this work with non-square weight matrices?]: 

\begin{equation}
h_{t} = \sum_{i=1}^t W^{t-i}Ux_{i} 
\end{equation}

This summation can be thought of as a filler-role representation, where the filler vector $x_i$ is bound to a role matrix $W^{t-i}U$. The important thing to note is that these role matrices are  using right-to-left roles; that is, for two sequences of different lengths, the fillers that have the same role matrices will be those that are the same distance from the end, not from the start. Thus, as this simplified case shows, right-to-left roles are actually very natural for a left-to-right network to adopt. Indeed, this fact may partly explain why, as observed by \cite{sutskever2014sequence}, reversing the order of the input is useful for sequence-to-sequence networks.
















